SSS3D: Fast Neural Architecture Search For Efficient Three-Dimensional Semantic Segmentation

We present SSS3D, a fast multi-objective NAS framework designed to find computationally efficient 3D semantic scene segmentation networks. It uses RandLA-Net, an off-the-shelf point-based network, as a super-network to enable weight sharing and reduce search time by 99.67% for single-stage searches. SSS3D has a complex search space composed of sampling and architectural parameters that can form 2.88 * 10^17 possible networks. To further reduce search time, SSS3D splits the complete search space and introduces a two-stage search that finds optimal subnetworks in 54% of the time required by single-stage searches.

==> data/S3DIS/Arch_1/gen1.tex <==
Error | Params
60.2129125912690 | 2.64722600000000
45.7212974167031 | 5.00759700000000

==> data/S3DIS/Arch_1/gen10.tex <==
Error | Params
78.2163822053320 | 2.20022700000000
56.4167426542277 | 2.20058300000000
55.3647190934801 | 2.43629600000000
44.4532353482590 | 2.70809300000000

==> data/S3DIS/Arch_1/gen15.tex <==
Error | Params
54.1453402141786 | 2.18841500000000
47.1223291203665 | 2.25074100000000
44.9593775563419 | 2.50963000000000
41.9235311409974 | 2.60309000000000
41.5806125714825 | 2.61603600000000
41.2592255786681 | 3.27453800000000

==> data/S3DIS/Arch_1/gen5.tex <==
Error | Params
85.6471900675033 | 2.49187500000000
78.8123742965603 | 2.49728900000000
76.2395908940739 | 2.55165100000000
65.2106342452914 | 2.70620200000000
61.8770014087842 | 2.79861300000000
52.1024558850411 | 2.88128000000000
50.3954511798527 | 3.99283600000000
49.2553744542015 | 4.53549000000000

==> data/S3DIS/Arch_2/gen1.tex <==
Error | Params
67.7511301233622 | 2.64722600000000
67.7435987359434 | 2.87552200000000
50.5900720911169 | 5.00759700000000

==> data/S3DIS/Arch_2/gen10.tex <==
Error | Params
81.2709259328477 | 2.17425100000000
52.1364472216939 | 2.49614700000000
51.4358825319738 | 2.55259800000000
44.9949182308046 | 2.60798800000000

==> data/S3DIS/Arch_2/gen15.tex <==
Error | Params
77.2967493899183 | 2.17157100000000
76.5444287993793 | 2.19016200000000
53.9575700417238 | 2.24290500000000
51.6708690188996 | 2.33175100000000
45.6506139745612 | 2.64774200000000

==> data/S3DIS/Arch_2/gen5.tex <==
Error | Params
53.6158577873091 | 2.25621600000000
53.0280100821323 | 2.91412400000000
50.4874085883876 | 4.57813600000000

==> data/S3DIS/Arch_3/gen1.tex <==
Error | Params
62.1353464283551 | 2.64722600000000
49.4160938527634 | 5.00759700000000

==> data/S3DIS/Arch_3/gen10.tex <==
Error | Params
59.6743084305541 | 2.26422100000000
54.9843893502352 | 2.41113300000000
48.0931023703060 | 2.64971100000000
45.8437095736202 | 2.83289700000000

==> data/S3DIS/Arch_3/gen15.tex <==
Error | Params
82.7415773737864 | 2.14787600000000
62.6852105875929 | 2.19065500000000
50.4917124488839 | 2.40819300000000
48.9785809139072 | 2.43415400000000
43.5238584207768 | 2.86332400000000

==> data/S3DIS/Arch_3/gen5.tex <==
Error | Params
77.9193402842418 | 2.20782100000000
74.9180933808600 | 2.54952100000000
70.8016428617886 | 2.56256700000000
60.0508626106371 | 3.22671700000000
50.2902021793077 | 3.59593100000000

==> data/S3DIS/Params/gen1.tex <==
Error | Params
92.4094612025343 | 2.98636000000000
45.9980 | 5.00759700000000

==> data/S3DIS/Params/gen10.tex <==
Error | Params
85.9091883332566 | 2.48647700000000
57.8295901787342 | 2.64641200000000
52.2845690100872 | 3.29635600000000

==> data/S3DIS/Params/gen20.tex <==
Error | Params
80.4410199007420 | 2.26775500000000
71.9704923977927 | 2.30478100000000
54.0224593012642 | 2.63853400000000
53.5521298004212 | 3.01334700000000
45.6611740147576 | 3.91141700000000
45.5182204035657 | 3.95972500000000
43.5710813517767 | 4.23777700000000

==> data/S3DIS/Params/gen30.tex <==
Error | Params
73.4458742140760 | 2.14936900000000
54.8581952396296 | 2.60764600000000
44.7151544922724 | 2.66384400000000
43.8535628240891 | 2.80621400000000
41.3111123539132 | 3.37238300000000
41.2418146098560 | 3.52758500000000

==> data/S3DIS/Params/gen40.tex <==
Error | Params
57.4273526818671 | 2.18338300000000
46.5211590081757 | 2.42089200000000

==> data/S3DIS/Params/gen50.tex <==
Error | Params
89.9449564348111 | 2.14791000000000
84.5358092984518 | 2.14824200000000
81.3116523817138 | 2.17388500000000
65.7049001937061 | 2.18451000000000
58.3141355124799 | 2.35560700000000
42.7100273147638 | 2.42089200000000
41.0055716438530 | 2.92703700000000
40.9537191867805 | 2.93643800000000

==> data/S3DIS/Params/gen59.tex <==
Error | Params
84.6209864111701 | 2.14807600000000
59.1715246528533 | 2.21643100000000
56.4995300248311 | 2.25537900000000
49.7641616861474 | 2.38750300000000
43.2829401433453 | 2.42089200000000
42.8467683713581 | 2.43596100000000
40.9775358745098 | 2.69538700000000
